Building blocks for complex tasks: Robust generative event extraction for radiology reports under domain shifts

This paper explores methods for extracting information from radiology reports that generalize across exam modalities to reduce requirements for annotated data. We demonstrate that multi-pass T5-based text-to-text generative models exhibit better generalization across exam modalities compared to approaches that employ BERT-based task-specific classification layers. We then develop methods that reduce the inference cost of the model, making large-scale corpus processing more feasible for clinical applications. Specifically, we introduce a generative technique that decomposes complex tasks into smaller subtask blocks, which improves a single-pass model when combined with multitask training. In addition, we leverage target-domain contexts during inference to enhance domain adaptation, enabling use of smaller models. Analyses offer insights into the benefits of different cost reduction strategies.

==> sections/abstract.tex <==
Radiology reports present findings and observations of radiologists, creating an unstructured textual representation of medical images. In this paper, we investigate the extraction of exam reason and findings from radiology reports when the exam modality varies during inference.  We demonstrate that T5-based text-to-text generative models exhibit better generalization across different exam modalities compared to approaches that employ BERT-based task-specific classification layers. Considering  generative methods often rely on large model sizes, we reduce inference costs by minimizing decoding passes and model sizes, thus making large-scale corpus processing more feasible for clinical applications. We introduce a novel generative technique that decomposes complex tasks into smaller subtask blocks, and decodes the subtask sequences in one pass. This reduces the compositionality gap and improves the reasoning with individual subtasks for more complex tasks using small models. To compensate for the limitations of smaller models, we leverage target-domain contexts during inference to enhance domain adaptation, making their performance comparable to larger models. Our findings offer valuable insights for developing robust and efficient generative models for event extraction.




==> sections/method.tex <==

\section{Method}

\subsection{Generative event extraction with T5}
\label{sec:method_t5}
%flow
% motivation (why use T5, use QA format for generalization capability, especially for rare child classes in the source domain,  BERT classifies on encoding and learn the tasks purely from the training data)
% T5 compared to BERT (model can leverage semantic meanings of input and output texts to understand the task )
% expand semantic meaining of T5: the entity or relation extraction will be present as prompt "what anatomies related to the trigger", the classification classes are represented in texts, ontology can help constrain the model in parent and child class hierachie. 
% flexibility in incorporating target-domain contexts


In order to improve the model's generalization capabilities over BERT-based alternatives \citep{radiology_kevin, spert}, we structured our event extraction task in a unified question-answering (QA) format \citep{Xie2022UnifiedSKGUA, t5}. By utilizing text-to-text formats for both inputs and outputs, the model leverages the semantic meanings of prompts for defining tasks and categorization labels. This proves particularly beneficial for long-tail imbalanced class label distributions, to reduce  limits of insufficient training examples  on rare classes within the source domain training data. Furthermore, the text-to-text format offers the flexibility to incorporate additional contexts  to facilitate tasks, as discussed in Section~\ref{sec:method_context}.


%input output text format: Input: the input prompt consists of the )(1) input sentence from clinical notes, (2) the question that describe the task, and (3) the ontology which provides the textual labels of classification tasks, and hiearychy relationship if multi-level granulaities are needed.  
%The output is to answer the questions for span and labels, for span detection the output will list the spans, and for classification, the output will contain the label in a bracket. When there are multiple types of subtasks, or multiple entities involved to be answered jointly, the output is a sequence of the answers.  To parse the results in post-preocessing, we use regular expression to parse the structure using template, and extracte entitie terms and their categories. To evaluate the event extraction where entities are matched at span-level, we need to use a converter to match to the terms in output to the spans in the input sentence. [details in appendix, for single token, we match the matched token .For multiple-token phrase, we match a phrase using the longest common in normlized string. Where there are multiple matches are found, we choose closets token to the start of the  for trigger, and the clcoste token to the query trigger.'

The input prompt comprises (1) an input sentence from clinical notes to extract events from, (2) a question that describes the task or  subtask, and (3) an ontology that provides textual labels for classification tasks and hierarchical relationships if multi-level granularities are required. 

This section describes \textbf{vanilla output formats} that answer for spans and labels for entities; for span detection, the output lists the spans, separated by comma symbols ",", while for classification, the output contains the label in brackets "[]". When different subtask types or multiple entities are involved and multiple subtasks need to be answered, the output is a sequence of subtask answers. In the post-processing phase, we employ regular expressions to extract entity terms and their respective categories, assuming that the prediction format remains consistent with the training data. To evaluate event extraction where entities are matched at the span level, we use a text-to-span converter to  locate the spans in the input sentences for the terms in the predictions. More details of the input and output formtas and the post-processing are in Appendix~\ref{sec:appendix_t5_prompt} and  Appendix~\ref{sec:appendix_post_processing} 

% pipeline approach
%We can run a pipeline approach that decode either in two-step or three step  to complete the 4 types of subtask in the whole event extraction tasks. Each pipeline compotnent is a  model are trained specialized for a subset of the subtask types. 

%The two step apporach invovles a first step for trigger span and trigger type classification, a second step for given each trigger, detecting the anatomy related to this trigger, including both anatomy spans and the anatomy normalization classes in parent and child levels. The three step apporach take an additional run for normalization for an given anatomy span, so each anatomy span are normalized individually.


One option for event extraction is to use a pipeline approach to address all types of subtasks in different steps. We present a two-step and three-step pipeline approaches as generative method baselines. Each step in the pipeline consists of a specialized model trained for a subset of the subtask types.

The two-step approach involves a first step for detecting trigger spans and trigger types, followed by a second step for identifying the anatomy associated with each detected trigger. This includes both detecting anatomy spans and normalizing anatomy at parent and child levels of anatomy categories. The three-step approach adds an additional step to the two-step method for normalizing of each identified anatomical entity individually. 


% joint approach: In the one-step joint approach, we merger all subtasks involves in the event extraction, that works for all four subtask types, and process multiple entities in one pass. This method will make the decoding sequence longer than seperate steps in the pipeline approach, and models are likely to perform worse than in the pieline method.


In the one-step joint extraction approach using \textbf{vanilla output formats}, we address all four types of subtasks, which may be associated with multiple entities, in a single pass per input sentence. This method results in longer output lengths compared to the individual steps within pipelines. Although this one-step approach reduces inference costs compared to pipelines, it is likely to negatively impact model performance due to the compositionality gap.



% We use T5 pretrained on medical and clinical domain. The prompts are listed in appendix [TODO prompts appendix]
 Our work build  generative models based one the clinical version of the T5 models \citep{clinicalt5}, which are pre-trained in medical literatures and clinical notes. This choice leverages their strengths in comprehending clinical text styles and medical knowledge.

\input{figures/figure1}

\subsection{Building blocks for subtasks}
%Motivatation: the event extracton can be viewed as multi-hop QA, involves a sequence of subtasks (trigger detection, trigger clafficiation, anatomy spand erection, anatomy normalziation). Merging steps can lead to compositionality gap,  and separate decoding, though helpful, in decoding time and diswanted for processing large-scale of notes.  We should composition gap could be even more severe when domain is changed and the relations to other subtasks drift more severely.


% Inspired by well generalizable HMM model, in which individual states and states transition are modeled separately, and we want to make the model solve at subtask separately and meanwhile learn the order of the sequence of subtasks to solve a complex task. By doing so, we help small models to show chain-of-thoughts ability at inference time.

Event extraction can be seen as a multi-hop question-answering (QA) process, involving a series of subtasks for successful completion. One-step decoding tends to experience performance decline under domain shifts, primarily due to the compositionality gap, which becomes more pronounced when transferring to a new domain with significantly altered subtask combinations. However, multiple decoding passes are not ideal due to high inference costs when processing large note collections.









Drawing inspiration from the versatile Hidden Markov Model (HMM), which concurrently models states and state transitions, our goal is to create a model that tackles subtasks individually and learns to sequence them for solving complex tasks. This approach aims to enable smaller models to display reasoning abilities previously demonstrated in LLMs \citep{chain-of-thought, self_ask}.


% [ what are the state prompts;  how to train with multitask. how to decode cheaply.]  unified distangle the tasks and  make each subtask output adjacent within themself, we change the prompt that structually encode the state of the task. In the output, the subtasks are enclosed into bloacks, and the whole tasks output can be viewed as a sequences of blocks corresponding to decomposed subtasks. In order to make subtask can be done in adjacent decoded segments within each block, and make the type of subtasks clear, we use a state to indicate the type of subtask, following the answer of the subtasks. We  expensively train in as subtasks as pipeline to learn substask indpendelty, and  one-step joint decoding which require undertan how to contrust subtasks sequences to solve the whole event extraction task.  In decoding, we decoding during inference in one-step to reduce inference costs. This is similar to self-ask \citep{self-ask}, the difference is they show subquestions in LLM, we enable small models here to follow subquestions. We show in small model senarios, the multitask training on subtasks is the key.


The vanilla output format in Section~\ref{} lacks clear subtask tracking and modularization, as answers are grouped by entities and concatenated by meaningless delimiters. To enhance this, we restructure the output by organizing answers into subtask blocks, incorporating explicit subtask state indicators. This approach enables decomposition of task outputs into independent subtasks while maintaining clear transitions between them.




We aggressively train the model on both entire tasks and their decomposed subtasks, resembles both the pipeline and one-step joint extraction approaches. This allows the model to perform subtasks independently and assemble subtask sequences for complex tasks. During inference, we decode in a single step to minimize costs. Our output format is similar to methods that perform reasoning steps in prompts for LLM \citep{chain-of-thought, self_ask},  but with a key distinction: we employ multitask training on individual subtasks, allowing smaller models to excel at simpler subquestions as reasoning steps. We demonstrate that this multitask training is crucial for the success of our method on small models.






\subsection{Incorporating target-domain contexts into prompts}
\label{sec:method_context}


%Motivatation: single input sentence can be subopitimal to have enoguht contexts for disambiguiation, and without addtiional resource reference to succeed in task, fortuantly the text format of input provide seamless incorporation for adding extra contexts to help tasks, even not require presence in training stage. The contexts will come from the target-domain to bias for target domain distribution. We specically use contexts to help the anatomy normalization as in section T5 anatomy normalization vanilla format. The contexts should be closely related to the anatomy information in the given input sentence, but provide some useful anatomy information that model can easily understand.

 %Desired contexts should describe the same anatomy part as the input sentence, and contain easier-to-understand anatomy information. (type of contexts) we use two type of contexts, document-level and domain-level contexts.   Document-level contexts include automatically extracted section headers and exam type metadata. Coming similar sentence make the document-level contexts likely to describe the relevant anatomy parts. section headers and exam type often summarize anatomy information. Domain-level contexts are from the target domain corpus, no annotations are required. We search for most similar sentence by lexcial match search algorithm BM25, the lexical match will make the retrieved sentence likely describe the same anatomy to the queried input sentece, and to make the retrieved sentencnes contain useful anatomy information that model can easily understand, we filtere the search scope to setnences that contain common anatomy terms that listed from anatomy noralzatiion categories and high frequency auto extracted section headers. 



%How: we only add contexts in decoding, the reason not to add it in training is because we want to avoid model learn source-domain specific reliance to the contexts. We test on a separate normalzation run: The reason to not directly added to one-step is longer contexts can mess up span detection because model may also extract spans from contexts intead of only from the input sentence.



A single input sentence may not provide enough information for a model to complete a task, as additional details may be needed for disambiguation or to supplement missing knowledge in pre-trained language models. Moreover, contexts from various domains can be heterogeneous, with missing values and distribution shifts. Fortunately, the text format of the input allows for the seamless integration of additional contexts from the target domain during inference to aid in the task and infuse helpful domain-specific bias, even if the models were not particularly trained for reading contexts. In our study, we specifically use contexts to assist in anatomy normalization, using the vanilla T5 format described in Section~\ref{sec:method_t5}. 

The desired contexts should be relevant the input sentence and contain helpful task information. We utilize two types of contexts - document-level and domain-level contexts to help anatomy normalization subtasks. Document-level contexts include automatically extracted section headers and exam type metadata associated with the same clinical note. The document-level contexts are likely to describe relevant anatomical parts, as section headers and exam types often summarize anatomy information. Domain-level contexts are retrieved from the unlabeled target-domain corpus.  We search for the most similar sentence with the greatest lexical overlap degree, using the search algorithm BM25. When the search pool is large, the top-ranked retrieved context sentence likely describes a similar anatomy part as the queried input sentence. To guarantee that the retrieved sentences also contain useful anatomy information that the model can easily understand, we narrow the search scope to 36\% to sentences containing common anatomy terms listed from anatomy normalization categories and high-frequency auto-extracted section headers.  We filter the corpus offline to speed up the search algorithm. See more details in Appendix~\ref{sec:appendix_context_retrieval}
%[TODO as listed in Appendix xx] [TODO statistics: after filtering, how many sentences are left]

%  unlabele PT data statistics
 % remove_punctuation(query).lower().strip().split(" ")
% we filter using the same BM25 model, but compare to anatomy string, and keep those with positive matching scores.
% filter for 50000 sentences with token number >3, from 1471 notes. after filter with anatomy terms, 51481 sentences are filtered to 18959, shrink to 36% of original size. 
% #'/home/sitongz/incidentalomas/analyses/step212_augment_meta_section_header/PT_100K/data_train.json'}

% data_unann = json.loads(open(domain_to_fn['PT_uann']).read())
% data_unann = [d for d in data_unann if len(d['tokens'])>3][:50000]
% # generate_count(data_unann)
% #{'note_ct': 1471, 'sent_ct': 50000} 
% after filter by anatomy
%     #51481 # 50000 uanna + PT test
    % #18959 #  bm25_anatomy_informative_scores>0
% Neurological:  Spine Cervical, Spine Thoracic, Spine Lumbar, Spine Sacral, Spine Cord, Spine , Brain, Nerve, Pituitary, \
% Cerebrospinal , Cerebrovascular, Extraaxial | \
% Cardiovascular:  Venous, Arterial, Pulmonary Artery, \
% Heart, Pericardial Sac, Coronary Artery \
% | Thoracic:  Mediastinal | Respiratory:  \
% Lung, Pleural Membrane, Tracheobronchial \
% | Digestive:  Esophagus, Stomach, Intestine,  Intestine,  Intestine \
% | Hepato-Biliary:  Gallblader, Bile , Pancreas, Liver \
% | Urinary:  Kidney, Urinary Bladder, Ureter \
% | Breast, Ovary, Uterus, Adnexal, Extra-embryonic, Placenta, Fetus, Umbilical Cord, \
% Genital Structure, Prostate, Testis, Epididymis \
% | Musculo-Skeletal:  Skeletal  Smooth Muscle, Bone   \
% |  Pelvis,  Limb \
% | Head Neck:  Thyroid, Neck, Ear, Eye, Mouth, Nasal Sinus, Pharynx, Laryngeal \
% | Skin: Skin  Mucous Membrane, Subcutaneous \
% | Abdomen:  Retroperitoneal, Abdominal , Peritoneal Sac, Spleen, Adrenal , Mesentery \
% |   Adipose , Chest, Mediastinum, Osseous, Bones, extremities, Lungs, MUSCULOSKELETAL, Ventricular, Bowel, Pleura, Spleen, Vasculature, Thorax, Gallbladder, Kidneys, Adrenals, Adrenal,Cardio \
% '


We only add contexts during decoding to prevent the model from relying too much on source-domain specific contexts. In the input prompts, exam type, section headers and prior sentences are placed before input sentences, following their natural orders. Other contexts are inserted between the input sentences and task ontology. We test this approach in a separate anatomy normalization run after the one-step joint decoding. The reason for not directly adding it to a one-step process is that introducing contexts to inputs can potentially corrupt span detection, as the model may extract spans from the context rather than exclusively from the input sentence. 




==> sections/results.tex <==
\input{tables/spert_vs_t5}


\section{Results}



%\subsection{Generative methods generalizes better under domain shifts}

\subsection{Benefit of generative model}

% Table~\ref{tab:main} presents in-domain and cross-domain results for different approaches. We observe a significant performance drop  for mSpERT models when moving from in-domain to cross-domain scenarios. The performance gap gets wider for anatomy parent (in-domain PET-PET 61.9 - cross-domain MR-PET 34.7\%) and child normalization tasks  (in-domain PET-PET 59.6, cross-domain MR-PET 33.5) when compared to trigger (82.4-75.6\%) and anatomy (65.8 - 59.9) extraction tasks  across domains. 

Table~\ref{tab:main} shows that \textbf{mSpERT models experience a significant performance drop in cross-domain scenarios compared to in-domain}. The gap is wider for anatomy normalization tasks. For the PET test set, the in-domain model's F1 score is 61.9\%, dropping to 34.7\% when trained on MRI. Similarly, the PET model scores 59.6\% on child normalization tasks, dropping to 33.5\% in the MRI cross-domain setting. In comparison,  when moving from in-domain PET to cross-domain MRI, span-level extraction decreases less, from 82.4\% to 75.6\% for trigger spans and 65.8\% to 59.9\% for anatomy spans. 






% When allowing no limits of the vanilla T5-base, the generative method outperforms mSpERT on both in-domain and out-domain settings, the gain is significant under great domain shifts. We use the maximum step in decoding, the three-step vanilla T5-base method, compared with mSpERT, the antomy parent score improve from 61.9  to 64.7 for in domain PET model, 47.5 to 53.3 for cross-domain CT model, and for the MRI model which suffers most cross-domain performance drop, the score improve from  34.7 to 48.6  by swtiching to the generative method.


When using unlimited decoding passes, \textbf{the T5-base generative method surpasses mSpERT in in-domain and out-domain settings}, and the improvements are significant under substantial domain shifts. With up to three-step decoding, T5-base pipeline raises anatomy parent-level normalization F1 scores from 61.9\% to 64.7\%  for the in-domain PET model, 47.5\% to 53.3\% for the cross-domain CT model, and most notably, from 34.7\% to 48.6\% for the cross-domain MRI model which suffers performance drop the most.





















\subsection{Benefit of subtask blocks}

% We demonstrate the compositionality gap in Table~\ref{tab:main}, where combining multiple steps in vanilla T5-base pipelines yields better performance than decoding with merged steps. For cross-domain generalization, the three-step vanilla T5-base models outperforms the vanilla two-step pipeline, which is better than the vanilla one-step joint approach. For instance, the cross-domain MRI model using vanilla three-step T5-base scores anatomy parent-level noralzation at 48.6\%, when reducing to two steps, the score drops to 47.1\%, and when only using one-step, the score is 44.9\%.   

Table~\ref{tab:main} shows that \textbf{combining multiple steps in vanilla T5-base methods leads to better performance than decoding with merged steps, referred to as the compositionality gap}. For cross-domain generalization, the vanilla three-step T5-base model outperforms the vanilla two-step, and the two-step one is better than the vanilla one-step joint approach. For example, in the cross-domain MRI model, the three-step T5-base achieves 48.6\% in anatomy parent-level normalization, while the two-step drops to 47.1\%, and the one-step scores at only 44.9\%. For in-domain evaluation, both multi-step pipelines surpass the one-step vanilla approach. The compositionality gap in parent-level anatomy normalization is more pronounced in cross-domain transfer than in-domain transfer. The vanilla three-step T5-base method improves in-domain performance from 63.3\% to 64.7\%, while the absolute gains for cross-domain models trained on MRI and CT source domains are around 5\% for each.






\textbf{Building subtask blocks improves the results of the single-step T5 method, particularly in terms of anatomy normalization performance}. The gains are substantial for the MRI source domain, in which the one-step anatomy parent-level normalization F1 score is improved from 44.9\% to 48.3\% after building subtasks blocks, nearly on-par with its three-step pipeline.





\subsection{Benefit from context incorporation}
\input{tables/context}


We add target-domain contexts to prompt during decoding to help anatomy normalization through a two-phase approach. First, we execute single-step decoding using the subtask block method with the T5-base model. Second, we categorize each identified anatomical span into normalized anatomy categories utilizing the vanilla T5 output format. 

For T5-base anatomy normalization models, (Table~\ref{tab:contexts}), \textbf{all types of contexts are beneficial under domain-shifts, with their combination often yielding better results}. T5-base's performance deteriorates compared to T5-large in the MRI domain, where domain-level contexts alone are comparable to T5-large and combined contexts outperform T5-large. However, in in-domain evaluations (PET to PET), domain-level information loses its usefulness, while document-level information remains helpful.

To explain, we observe that contexts assist in disambiguation and provide hints for difficult medical terms (Example in Appendix~\ref{sec:appendix_case_study}). Disambiguation often requires same-document contexts, while hints for challenging examples are more likely collected from a large domain-level corpus rather than just the same document. This might explain why in-domain models (PET) benefit more from document-level contexts for disambiguation, whereas the cross-domain model,  that lacks target-domain medical knowledge (MRI), benefit more from domain-level contexts.

% As demonstrated in Table~\ref{tab:contexts}, both document-level and domain-level contexts empower the T5-base model to be comparable to the more expansive T5-large model.  In MRI to PET transfer scenario where the performance gap between small and large models is greater than in other scenarios, the domain-level contexts make T5-base model comparable T5-large model on child-level normalization, and even better on the parent level.



==> tables/TODO_stats_corpus_filtered_size.tex <==
\begin{table}[h!]
\centering
\begin{tabular}{@{}lrr@{}}
\toprule
\textbf{Domain} & \multicolumn{1}{l}{\textbf{Note \#}} & \multicolumn{1}{l}{\textbf{Sent \#}} \\ \midrule
CT\_train        & 143                                   & 3707                                 \\
MR\_train        & 144                                   & 3551                                 \\
PT\_train        & 142                                   & 5184                                 \\
PT\_dev          & 20                                    & 758                                  \\
PT\_test         & 40                                    & 1481                                 \\ \bottomrule
\end{tabular}
\caption{Ordered data table}
\label{tab:my_label}
\end{table}

==> tables/cost_inference.tex <==
\begin{table}[ht]
\centering
\caption{\textcolor{red}{Number of inference instances of one-step and multi-step approaches. We report the pipeline trained on the MRI domain and tested on the PET domain. The decoding passes per sample are the average of runs among 1481 test-set samples, and the token counts per sample are the average of the sum of input and output token counts. The first three rows are the same as in Table~\ref{tab:main}, and the last row is the same as the "T5-base 
all
combined" column in the Table~\ref{tab:contexts}  }}
\label{tab:cost_inference}
\renewcommand{\arraystretch}{0.8} % This is where the line spacing is set. Adjust as needed.
\begin{tabularx}{\columnwidth}{@{}>{\hsize=1.4\hsize}X*{2}{>{\centering\arraybackslash\hsize=0.8\hsize}X}@{}}
\toprule
\textbf{Method} & \textbf{decoding passes per sample} & \textbf{token counts per sample} \\ \midrule
T5-base three-step (vanilla) & 2.5 & 0.36 K \\
T5-base two-step (vanilla) & 1.7 & 0.2 K \\
T5-base one-step (blocks) & 1 & 0.25 K \\
 T5-base one-step
(blocks) \\ + normalization with contexts all
combined  & 1.7 & 0.45 K \\
\bottomrule
\end{tabularx}
\end{table}



% \begin{table}[ht]
% \centering
% \caption{\textcolor{red}{Number of inference instances of one-step and multi-step approaches. We report the pipeline trained on the MRI domain and tested on the PET domain.}}
% \label{tab:cost_inference}
% \begin{tabularx}{\columnwidth}{@{}>{\hsize=.8\hsize}X*{1}{>{\centering\arraybackslash\hsize=1.06666\hsize}X}@{}}
% \toprule
% \textbf{Method} & \textbf{Number of Inference Instances} \\ \midrule
% T5-base three-step
% (vanilla) & 3644 \\
% T5-base two-step
% (vanilla)& 2585 \\
% T5-base one-step 
% (blocks) & 1481 \\
% \bottomrule
% \end{tabularx}
% \end{table}

==> tables/spert_vs_t5_old.tex <==

\begin{table*}[ht]
\centering
\caption{Generative approach is better under domain shifts. Compositionality gap when decoding in merged steps. Building subtasks blocks for one-step decoding. }
\label{tab:main}
\begin{tabularx}{\textwidth}{@{}l*{6}{>{\centering\arraybackslash}X}@{}}
\toprule

%PT (2-step, 3-step, , 1-step)
% 0.819	0.819	0.821
% 0.676	0.676	0.660
% 0.649	0.647	0.633
% 0.623	0.621	0.597
%multitask
% 0.826
% 0.661
% 0.635
% 0.607
\textbf{Entity} & \textbf{mSpERT} & \textbf{T5-large three-step ( DELETE )} & \textbf{T5-base three-step vanilla} & \textbf{T5-base two step vanilla} & \textbf{T5-base one-step vanilla} & \textbf{T5-base one-step (building blocks)} \\ \midrule
& \multicolumn{6}{c}{\textbf{PET → PET}} \\ \cmidrule(lr){2-7}
Trigger & 82.4 & -- & 81.9 & 81.9 & 82.1 & 82.6 \\
Anatomy & 65.8 & -- & 67.6 & 67.6 & 66.0 & 66.1 \\
Anatomy Parent & 61.9 & -- & 64.7  & 64.9 & 63.3 & 63.5 \\
Anatomy Child & 59.6 & -- & 62.1 & 62.3 & 59.7 & 60.7 \\
 \midrule
& \multicolumn{6}{c}{\textbf{MRI → PET}} \\ \cmidrule(lr){2-7}

Trigger & 75.6 & 76.9xx & 76.6 & 76.6 & 76.4 & 77.8 \\
Anatomy & 59.9 & 62.5xx & 60.9 & 60.9 & 59.2 & 61.1 \\
Anatomy Parent & 34.7 & 49.1xx & 48.6  & 47.1 & 44.9 & 48.3 \\
Anatomy Child & 33.5 & 49.9xx & 44.6 & 44.0 & 41.2 & 44.8 \\
 \midrule
& \multicolumn{6}{c}{\textbf{CT → PET}} \\ \cmidrule(lr){2-7}

Trigger & 75.7 & -- &76.1 & 76.1 & 74.0 & 76.6 \\
Anatomy & 59.7 & -- & 61.4	 & 61.4 & 56.3 & 59.8 \\
Anatomy Parent & 53.2 & -- &  55.8 & 54.8 & 50.8 & 55.0 \\
Anatomy Child & 47.5 & -- & 53.3 & 51.8 & 48.1 & 51.2 \\
\bottomrule
\end{tabularx}
\end{table*}

%CT (2-step, 3-step, , 1-step)
% 0.761	0.761	0.740
% 0.614	0.614	0.563
% 0.548	0.558	0.508
% 0.518	0.533	0.481

% 0.733
% 0.568
% 0.521
% 0.488
% CT multitask_with_anatomy_span
% 0.766
% 0.598
% 0.550
% 0.512
